Coordinating Stakeholders in the Consideration of Performance Indicators and Respective Interface Requirements for Automated Vehicles

This paper presents a process for coordinating stakeholders in their consideration of performance indicators and respective interface requirements for automated vehicles. These performance indicators are obtained and processed based on the system's self-perception and enable the realization of self-aware and self-adaptive vehicles. This is necessary to allow SAE Level 4 vehicles to handle external disturbances as well as internal degradations and failures at runtime. Without such a systematic process for stakeholder coordination, architectural decisions on realizing self-perception become untraceable and effective communication between stakeholders may be compromised. Our process-oriented approach includes necessary ingredients, steps, and artifacts that explicitly address stakeholder communication, traceability, and knowledge transfer through clear documentation. Our approach is based on the experience gained from applying the process in the autotech.agil project, from which we further present lessons learned, identified gaps, and steps for future work.

==> content/0_abstract.tex <==
%%% Abstract
\begin{abstract}
%
% 138 words
%
This paper presents a process for coordinating stakeholders in their consideration of performance indicators and respective interface requirements for automated vehicles. These performance indicators are obtained and processed based on the system's \selfp and enable the realization of \saw and \sad vehicles. This is necessary to allow SAE Level 4 vehicles to handle external disturbances as well as internal degradations and failures at runtime. Without such a systematic process for stakeholder coordination, architectural decisions on realizing \selfp become untraceable and effective communication between stakeholders may be compromised. Our process-oriented approach includes necessary ingredients, steps, and artifacts that explicitly address stakeholder communication, traceability, and knowledge transfer through clear documentation. Our approach is based on the experience gained from applying the process in the \autotech project, from which we further present lessons learned, identified gaps, and steps for future work.
%
\end{abstract}

==> setup/authors.tex <==
\newcommand{\yearstring}{2025}
\newcommand{\bibstring}{tbd}
\newcommand{\conferencestring}{}
\newcommand{\addressstring}{}

% Author block offset variables
\newcommand{\OffsetForInsertFiveAuthorsFirstAuthor}{-2.5cm}
\newcommand{\OffsetForInsertFiveAuthorsSecondAuthor}{-0.5cm}
\newcommand{\OffsetForInsertFiveAuthorsThirdAuthor}{-0.5cm}
\newcommand{\OffsetForInsertFiveAuthorsFourthAuthor}{3cm}
\newcommand{\OffsetForInsertFiveAuthorsFifthAuthor}{0cm}

% Author block offset variables for six authors (3+3 layout)
% First row: 3 authors evenly spaced
\newcommand{\OffsetForInsertSixAuthorsFirstAuthor}{-2.2cm}
\newcommand{\OffsetForInsertSixAuthorsSecondAuthor}{-0.5cm}
\newcommand{\OffsetForInsertSixAuthorsThirdAuthor}{-0.5cm}
% Second row: 3 authors evenly spaced (aligned with first row, reset to start of line)
\newcommand{\OffsetForInsertSixAuthorsFourthAuthor}{0cm}
\newcommand{\OffsetForInsertSixAuthorsFifthAuthor}{6.0cm}
\newcommand{\OffsetForInsertSixAuthorsSixthAuthor}{1.5cm}
% Vertical space variables for authors 5 and 6
\newcommand{\VspaceForInsertSixAuthorsFifthAuthor}{-3.08cm}
\newcommand{\VspaceForInsertSixAuthorsSixthAuthor}{-3.11cm}

% E-Mails
\newcommand{\emailOne}{richard.schubert@tu-bs.de}
\newcommand{\emailTwo}{m.loba@tu-bs.de}
\newcommand{\emailThree}{kluener@embedded.rwth-aachen.de}
\newcommand{\emailFour}{alexander.bloedel@tu-darmstadt.de}
\newcommand{\emailFive}{kampmann@embedded.rwth-aachen.de}
\newcommand{\emailSix}{steven.peters@fzd.tu-darmstadt.de}

% Variables for author information
\newcommand{\AuthorOneName}{Richard Schubert}
\newcommand{\AuthorOneInstOne}{Institute for Control Engineering}
\newcommand{\AuthorOneInstTwo}{TU Braunschweig}
\newcommand{\AuthorOneCity}{Braunschweig, Germany}
\newcommand{\AuthorOneEmail}{\emailOne}

\newcommand{\AuthorTwoName}{Marvin Loba}
\newcommand{\AuthorTwoInstOne}{Institute for Control Eng.}
\newcommand{\AuthorTwoInstTwo}{TU Braunschweig}
\newcommand{\AuthorTwoCity}{Braunschweig, Germany}
\newcommand{\AuthorTwoEmail}{\emailTwo}

\newcommand{\AuthorThreeName}{Alexander Blödel}
\newcommand{\AuthorThreeInstOne}{Institute of Automotive Engineering}
\newcommand{\AuthorThreeInstTwo}{TU Darmstadt}
\newcommand{\AuthorThreeCity}{Darmstadt, Germany}
\newcommand{\AuthorThreeEmail}{\emailFour}

\newcommand{\AuthorFourName}{David Klüner}
\newcommand{\AuthorFourInstOne}{Chair of Embedded Software}
\newcommand{\AuthorFourInstTwo}{RWTH Aachen University}
\newcommand{\AuthorFourCity}{Aachen, Germany}
\newcommand{\AuthorFourEmail}{\emailThree}

\newcommand{\AuthorFiveName}{Alexandru Kampmann}
\newcommand{\AuthorFiveInstOne}{Chair of Embedded Software}
\newcommand{\AuthorFiveInstTwo}{RWTH Aachen University}
\newcommand{\AuthorFiveCity}{Aachen, Germany}
\newcommand{\AuthorFiveEmail}{\emailFive}

\newcommand{\AuthorSixName}{Steven Peters}
\newcommand{\AuthorSixInstOne}{Institute of Automotive Eng.}
\newcommand{\AuthorSixInstTwo}{TU Darmstadt}
\newcommand{\AuthorSixCity}{Darmstadt, Germany}
\newcommand{\AuthorSixEmail}{\emailSix}

% Command to insert five authors (no arguments - uses variables defined above)
\newcommand{\insertFiveAuthors}{%
\author{%
\ifisanonymized
% Anonymized version: show black box with same height
\rule{\textwidth}{\AnonymizedAuthorsHeight}
\else
% Normal version: show actual authors
\IEEEauthorblockN{\hspace{\OffsetForInsertFiveAuthorsFirstAuthor}\AuthorOneName}
\IEEEauthorblockA{\hspace{\OffsetForInsertFiveAuthorsFirstAuthor}\textit{\AuthorOneInstOne} \\
\hspace{\OffsetForInsertFiveAuthorsFirstAuthor}\textit{\AuthorOneInstTwo}\\
\hspace{\OffsetForInsertFiveAuthorsFirstAuthor}\AuthorOneCity \\
\hspace{\OffsetForInsertFiveAuthorsFirstAuthor}\AuthorOneEmail}
\and
\IEEEauthorblockN{\hspace{\OffsetForInsertFiveAuthorsSecondAuthor}\AuthorTwoName}
\IEEEauthorblockA{\hspace{\OffsetForInsertFiveAuthorsSecondAuthor}\textit{\AuthorTwoInstOne} \\
\hspace{\OffsetForInsertFiveAuthorsSecondAuthor}\textit{\AuthorTwoInstTwo}\\
\hspace{\OffsetForInsertFiveAuthorsSecondAuthor}\AuthorTwoCity \\
\hspace{\OffsetForInsertFiveAuthorsSecondAuthor}\AuthorTwoEmail}
\and
\IEEEauthorblockN{\hspace{\OffsetForInsertFiveAuthorsThirdAuthor}\AuthorThreeName}
\IEEEauthorblockA{\hspace{\OffsetForInsertFiveAuthorsThirdAuthor}\textit{\AuthorThreeInstOne} \\
\hspace{\OffsetForInsertFiveAuthorsThirdAuthor}\textit{\AuthorThreeInstTwo}\\
\hspace{\OffsetForInsertFiveAuthorsThirdAuthor}\AuthorThreeCity \\
\hspace{\OffsetForInsertFiveAuthorsThirdAuthor}\AuthorThreeEmail}
\and
\IEEEauthorblockN{\hspace{\OffsetForInsertFiveAuthorsFourthAuthor}\AuthorFourName}
\IEEEauthorblockA{\hspace{\OffsetForInsertFiveAuthorsFourthAuthor}\textit{\AuthorFourInstOne} \\
\hspace{\OffsetForInsertFiveAuthorsFourthAuthor}\textit{\AuthorFourInstTwo}\\
\hspace{\OffsetForInsertFiveAuthorsFourthAuthor}\AuthorFourCity \\
\hspace{\OffsetForInsertFiveAuthorsFourthAuthor}\AuthorFourEmail}
\and
\IEEEauthorblockN{\hspace{\OffsetForInsertFiveAuthorsFifthAuthor}\AuthorFiveName}
\IEEEauthorblockA{\hspace{\OffsetForInsertFiveAuthorsFifthAuthor}\textit{\AuthorFiveInstOne} \\
\hspace{\OffsetForInsertFiveAuthorsFifthAuthor}\textit{\AuthorFiveInstTwo}\\
\hspace{\OffsetForInsertFiveAuthorsFifthAuthor}\AuthorFiveCity \\
\hspace{\OffsetForInsertFiveAuthorsFifthAuthor}\AuthorFiveEmail}
\fi
}%
}

% Command to insert six authors (no arguments - uses variables defined above)
\newcommand{\insertSixAuthors}{%
\author{%
\ifisanonymized
% Anonymized version: show black box with same height
\rule{\textwidth}{\AnonymizedAuthorsHeight}
\else
% Normal version: show actual authors
\IEEEauthorblockN{\hspace{\OffsetForInsertSixAuthorsFirstAuthor}\AuthorOneName}
\IEEEauthorblockA{\hspace{\OffsetForInsertSixAuthorsFirstAuthor}\textit{\AuthorOneInstOne} \\
\hspace{\OffsetForInsertSixAuthorsFirstAuthor}\textit{\AuthorOneInstTwo}\\
\hspace{\OffsetForInsertSixAuthorsFirstAuthor}\AuthorOneCity \\
\hspace{\OffsetForInsertSixAuthorsFirstAuthor}\AuthorOneEmail}
\and
\IEEEauthorblockN{\hspace{\OffsetForInsertSixAuthorsSecondAuthor}\AuthorTwoName}
\IEEEauthorblockA{\hspace{\OffsetForInsertSixAuthorsSecondAuthor}\textit{\AuthorTwoInstOne} \\
\hspace{\OffsetForInsertSixAuthorsSecondAuthor}\textit{\AuthorTwoInstTwo}\\
\hspace{\OffsetForInsertSixAuthorsSecondAuthor}\AuthorTwoCity \\
\hspace{\OffsetForInsertSixAuthorsSecondAuthor}\AuthorTwoEmail}
\and
\IEEEauthorblockN{\hspace{\OffsetForInsertSixAuthorsThirdAuthor}\AuthorThreeName}
\IEEEauthorblockA{\hspace{\OffsetForInsertSixAuthorsThirdAuthor}\textit{\AuthorThreeInstOne} \\
\hspace{\OffsetForInsertSixAuthorsThirdAuthor}\textit{\AuthorThreeInstTwo}\\
\hspace{\OffsetForInsertSixAuthorsThirdAuthor}\AuthorThreeCity \\
\hspace{\OffsetForInsertSixAuthorsThirdAuthor}\AuthorThreeEmail}
\and[\\]
\IEEEauthorblockN{\hspace{\OffsetForInsertSixAuthorsFourthAuthor}\AuthorFourName}
\IEEEauthorblockA{\hspace{\OffsetForInsertSixAuthorsFourthAuthor}\textit{\AuthorFourInstOne} \\
\hspace{\OffsetForInsertSixAuthorsFourthAuthor}\textit{\AuthorFourInstTwo}\\
\hspace{\OffsetForInsertSixAuthorsFourthAuthor}\AuthorFourCity \\
\hspace{\OffsetForInsertSixAuthorsFourthAuthor}\AuthorFourEmail}
\and
\IEEEauthorblockN{\vspace{\VspaceForInsertSixAuthorsFifthAuthor}}
\IEEEauthorblockA{\hspace{\OffsetForInsertSixAuthorsFifthAuthor}
{\normalfont{\sffamily}\sublargesize\AuthorFiveName} \\
\hspace{\OffsetForInsertSixAuthorsFifthAuthor}\textit{\AuthorFiveInstOne} \\
\hspace{\OffsetForInsertSixAuthorsFifthAuthor}\textit{\AuthorFiveInstTwo}\\
\hspace{\OffsetForInsertSixAuthorsFifthAuthor}\AuthorFiveCity \\
\hspace{\OffsetForInsertSixAuthorsFifthAuthor}\AuthorFiveEmail}
\and
\IEEEauthorblockN{\vspace{\VspaceForInsertSixAuthorsSixthAuthor}}
\IEEEauthorblockA{\hspace{\OffsetForInsertSixAuthorsSixthAuthor}
{\normalfont{\sffamily}\sublargesize\AuthorSixName} \\
\hspace{\OffsetForInsertSixAuthorsSixthAuthor}\textit{\AuthorSixInstOne} \\
\hspace{\OffsetForInsertSixAuthorsSixthAuthor}\textit{\AuthorSixInstTwo}\\
\hspace{\OffsetForInsertSixAuthorsSixthAuthor}\AuthorSixCity \\
\hspace{\OffsetForInsertSixAuthorsSixthAuthor}\AuthorSixEmail}
\fi
}%
}

==> setup/tweaks.tex <==

\newcommand{\OffsetTitleToAuthors}{-0.275cm}
\newcommand{\OffsetAuthorsToAbstract}{-1.45cm}

% Height variables for anonymization boxes
% Authors block height (full page width, 2 rows of authors)
\newcommand{\AnonymizedAuthorsHeight}{4.5cm}
% Research grant info height (footer/column width)
\newcommand{\AnonymizedGrantInfoHeight}{0.9cm}
% Additional vertical space after grant info box to prevent text overlap
\newcommand{\AnonymizedGrantInfoExtraSpace}{0.4cm}
% Acknowledgement section height (column width)
\newcommand{\AnonymizedAcknowledgementHeight}{0.5cm}
%
% Reduce space between authors and abstract
\ifisanonymized
\IEEEaftertitletext{\vspace{\OffsetAuthorsToAbstract}\vspace{\AnonymizedGrantInfoExtraSpace}}
\else
\IEEEaftertitletext{\vspace{\OffsetAuthorsToAbstract}}
\fi

% Rename sections autoref
\def\sectionautorefname{Section}
\def\subsectionautorefname{Subsection}
\def\figureautorefname{Fig.}
\def\tableautorefname{Table}

% Footnote Rule
\def\footnoterule{\hrule\vspace{1mm}}

% Reduce whitespace above footnote
\setlength{\skip\footins}{0.35\skip\footins}

% Reduce whitespace before and after figures
\setlength{\textfloatsep}{0.1\textfloatsep}

% Reduce whitespace before and after tables
\setlength{\floatsep}{0.1\floatsep}

% Adjust the spacing before sections
\newcommand{\titlebaselineskip}{0.25\baselineskip}
\titlespacing*{\section}{-0.75em}{\dimexpr\titlebaselineskip}{\titlebaselineskip}

% Reduce math equation whitespace before and after
\newcommand{\eqskipInPt}{5pt}
\AtBeginDocument{%
  \abovedisplayskip=\eqskipInPt
  \abovedisplayshortskip=\eqskipInPt
  \belowdisplayskip=\eqskipInPt
  \belowdisplayshortskip=\eqskipInPt
}

% Fix paragraph format
% \titleformat{\paragraph}[runin]{\normalfont\normalsize\itshape}{\theparagraph}{0.5em}{\hspace{0.5em}}[:]
% \titlespacing*{\paragraph}{0pt}{1ex plus 0.5ex minus 0.2ex}{0.5em}
% \renewcommand{\theparagraph}{\alph{paragraph})}

% Reduce the font size of the bibliography
% \setlength{\bibitemsep}{-0.1\baselineskip} % Between the items
\renewcommand*{\bibfont}{\fontsize{8}{9}\selectfont}

% Between the enumeration and the item, reduce the horizontal space
\setlength{\biblabelsep}{0.825\labelsep}

% Quote environment
\renewenvironment{quote}
  {\vspace{0.15em}\list{}{\rightmargin=10pt \leftmargin=10pt}%
   \item\relax}
  {\endlist\vspace{0.15em}}
